Pricing Pandora's Boxes: Revenue Maximization in Sequential Information Acquisition

We study a mechanism design problem in which a seller controls access to information about a set of stochastic alternatives, and a buyer sequentially acquires information in order to choose a single alternative with high value. The value distributions of the alternatives are known to both parties. The seller posts non adaptive prices for revealing each alternative's realized value, and the buyer responds optimally by following a Pandora's Box strategy: deciding which alternatives to inspect and when to stop by accepting the best inspected alternative. The seller's goal is to maximize his expected revenue, i.e. the total payment collected from all inspections. We study the revenue objective through the lens of simplicity versus optimality. Our main result is that a simple and efficiently computable pricing scheme obtains a 4 approximation in the worst case to the optimal revenue. This pricing rule equalizes the Weitzman indices across all alternatives. In contrast, we show that equalizing the prices themselves can be an unbounded factor worse than the optimum. Furthermore, for several natural special cases, including identically distributed alternatives and monotone hazard rate distributions, we fully characterize the optimal pricing. Finally, we also study a variant of our model under optional inspection, where the buyer may select an alternative without observing its realization. In this setting, we obtain an n/(n-1) approximation for the special case of n identically distributed alternatives, as well as a 2 approximation for the special case where each alternative's value distribution has support size two. Overall, our results highlight both the computational challenges and the power of simple pricing schemes in selling information to a sequential searcher.

==> old_intro.tex <==
\section{Introduction}

A company planning to launch a new product must often choose among several potential markets. Each market differs in its size, competitive landscape, regulatory environment, and consumer demand, all of which determine the eventual profitability of entering that market. To inform this decision, the company may hire a market research firm to estimate the net value of launching in each market. After gathering some information, the company intends to select a single market in which to launch, aiming to maximize its eventual profit.

We view this situation from the perspective of the market research firm. How should it sell its services? Should it charge more for reports about more promising markets? Should it encourage broad exploration or targeted investigation? And how should prices be set knowing that the company will decide sequentially which markets to investigate and may stop early once it finds a sufficiently attractive option?

A similar question arises in hiring. A recruiter evaluating multiple candidates may rely on a background-check provider to screen applicants. Each report reveals potentially valuable information about a candidate's suitability, but generating such reports is costly. How should the background-check provider price reports for individual candidates, given that the recruiter will choose whom to investigate and ultimately hire only one person?

These examples share a common structure: a buyer seeks to identify the best among several alternatives, while a seller controls access to information about those alternatives and can charge for its disclosure.

We formalize this interaction as a pricing problem for a Pandora’s Box searcher. There is a single seller with access to information about a collection of stochastic alternatives, and a single buyer who wishes to select the alternative with the highest realized value. The seller sets prices for revealing information about each alternative. Anticipating these prices, the buyer chooses an order in which to inspect alternatives, pays to reveal their realizations, and stops at some point to select the best option observed so far.

The buyer’s behavior is governed by a Pandora's Box strategy: a sequential search policy that trades off the expected benefit of further information against its cost. The seller's problem is to choose prices that maximize expected revenue, taking into account the buyer's optimal search behavior.

The problem of selling information has been studied extensively under the umbrella of information design and Bayesian persuasion (see, e.g., Bergemann and Morris). In that literature, an information provider observes the full state of the world and designs arbitrary signals—possibly complex and correlated—to influence a decision maker's actions.

Our focus is different. We study a more structured and operational setting in which the signals are fixed in advance and correspond directly to the buyer’s search problem. Each signal reveals the realized value of a specific alternative. The seller does not design new signals or garble information; instead, their only lever is pricing. This restriction reflects many real-world contexts, such as market research reports or background checks, where the form of the information is largely predetermined and the strategic question is how to price access to it. This structure allows us to isolate the economic and algorithmic aspects of pricing information when buyers engage in sequential search.

Formally, there are $n$ stochastic alternatives $X_1, \dots, X_n$ drawn from a known joint prior shared by both buyer and seller. The seller commits to and publicly announces a price $p_i\in [0, \infty]$ for observing and revealing the realization of $X_i$. The buyer may then pay $p_i$ to observe $X_i$ in any order of their choosing. After observing some subset of alternatives, the buyer may stop and select one alternative, obtaining its realized value. The seller’s revenue is the sum of prices paid for all revealed alternatives. The buyer is rational and chooses a search and stopping strategy that maximizes expected utility given the announced prices.

To illustrate the basic tension, consider a setting with two options: one stochastic alternative $X$ and one outside option with known value $v$. How much can the seller charge to reveal $X$? If the buyer must inspect an option before selecting it, then revealing $X$ has value only insofar as it improves upon $v$. In this case, the seller’s optimal price is tied to the expected surplus $E[(X-v)^+]$, since the buyer will pay at most that amount to learn whether $X$ beats the known alternative. By contrast, if the buyer is allowed to select an option without inspecting it, the calculus changes. The buyer may commit to 
$X$ ex ante, making the option to inspect less valuable and weakening the seller’s pricing power. Make the example precise and add some numbers. This distinction highlights how inspection rules shape the incentives and feasible revenue of the seller.

These two variants--optional and mandatory inspection--capture different real-world scenarios. In hiring or housing markets, inspections such as background checks or home inspections may be mandatory before a final decision is made. In contrast, in market research or product testing, firms may choose to act on partial information or forgo certain analyses altogether. From the buyer's perspective, these settings induce different search problems. Mandatory inspection leads to a classic Pandora's Box formulation with reservation values and optimal stopping rules. Optional inspection introduces additional complexity, as the buyer's problem becomes computationally hard. As a result, the seller’s pricing problem differs substantially between the two models, and both are economically meaningful.

\paragraph{Selling mechanisms.}
At one extreme, if the seller were allowed to bundle information—revealing all realizations at a single take-it-or-leave-it price—then the seller could extract the buyer’s entire expected surplus. Such full extraction is well understood in information design settings and relies on offering the buyer a perfectly tailored signal. (Check this and find refs.)
This outcome, however, runs counter to the spirit of the pricing problem we study. We therefore restrict attention to itemized pricing: each alternative must be priced individually, and the buyer chooses which pieces of information to acquire. Moreover, prices are non-adaptive and announced upfront, before the buyer begins searching.

Within this framework, we allow the seller to set prices of zero, revealing some information for free, as well as prices of infinity, effectively withholding certain information altogether. Our goal is to understand how much revenue a seller can extract under these natural and practically motivated constraints, and to design approximately optimal pricing schemes for this setting.

\paragraph{Our results.} TBD

Some further directions:
- what if the seller faces costs?
- what if the buyer wants to buy k things or ? 

